Fake Sentence Detection as a Training Task for Sentence Encoding

Sentence encoders are typically trained on language modeling tasks with large unlabeled datasets. While these encoders achieve state-of-the-art results on many sentence-level tasks, they are difficult to train with long training cycles. We introduce fake sentence detection as a new training task for learning sentence encoders. We automatically generate fake sentences by corrupting original sentences from a source collection and train the encoders to produce representations that are effective at detecting fake sentences. This binary classification task turns to be quite efficient for training sentence encoders. We compare a basic BiLSTM encoder trained on this task with a strong sentence encoding models (Skipthought and FastSent) trained on a language modeling task. We find that the BiLSTM trains much faster on fake sentence detection (20 hours instead of weeks) using smaller amounts of data (1M instead of 64M sentences). Further analysis shows the learned representations capture many syntactic and semantic properties expected from good sentence representations.

==> intro.tex <==
\section{Introduction}

Unsupervised sentence encoders are often trained on language modeling based tasks where the encoded sentence representations are used to reconstruct the input sentence~\cite{hill2016learning} or generate neighboring sentences~\cite{kiros2015skip,hill2016learning}. The trained encoders produce sentence representations that achieve the best performance on many sentence-level prediction tasks~\cite{hill2016learning}.
%This enables encoders to create representations such that sentences that similar in meaning or topic are closer in the embedded space. The trained representations achieve the best performance on many sentence-level prediction tasks~\cite{hill2016learning}.

However, this language modeling based training is problematic in two respects: 1) Training a language model to predict over larger contexts (neighboring sentences) requires large amounts of training data and time. Predicting neighboring sentences is a difficult and under-constrained task as there can be many valid possibilities for nearby sentences for any particular input sentence. 2) There is nothing explicit in the training task to force the encoder to learn fine grained distinctions between sentences that are mostly similar, a requirement often needed in downstream applications such as natural language inference (NLI).

In this paper we introduce an unsupervised discriminative training task, {\em fake sentence detection}, which is aimed at learning representations that distinguish sentences that are mostly similar in their words but may differ significantly in meaning or structure. The main idea is to generate fake sentences by corrupting an original sentence. We use two methods to generate fake sentences:  {\em word shuffling} where we swap the positions of two words at random and {\em word dropping}, where we drop a word at random from the original sentence.

This training task formulation has two key advantages:
(i) Corrupting a sentence can lead to break in syntactic coherence (e.g. missing a verb) leading to a malformed sentence or can cause a big change in the semantics (e.g., swapping subjects with object can be relevant for NLI) or a minor but meaningful distinction (e.g., dropping an adjective can be relevant for sentiment). In extremely rare cases the meaning may not change at all. Given that the sentences are going to be mostly similar (every pair is within a edit distance of two), for the encoder to be successful it must learn to tease apart the compositional aspects of meaning and explicitly learn to detect these small but meaningful shifts.
(ii) This binary classification task can be modeled with fewer parameters in the output layer and can be trained more efficiently compared to the language modeling training tasks where the output layer has many parameters depending on the vocabulary size.
%\minh{Is the input to the classifier is a pair of sentences instead of a single sentence? If the input is a pair of sentence and you use drop-word model, would it always be true to output the shorter sentence as fake? Is the learned representation biased toward short/long sentence?}


Given a large unlabeled corpus, for every original sentence, we add multiple fake sentences. The training task is then to take any given sentence as input and predict whether it is a real or fake sentence.
We train a bidirectional long short term memory network (BiLSTM) encoder that produces a representation of the input sentence, which is then used by a three-layer feed-forward network for prediction. We then evaluate this trained encoder {\em without any further tuning} on multiple sentence-level tasks and test for syntactic and semantic properties which demonstrate the benefits of fake sentence training. 


%Our evaluation shows that the BiLSTM model trained on fake sentence detection outperforms strong baselines trained on a much larger portion of the same corpus for language modeling tasks (FastSent~\cite{hill2016learning} and Skipthought~\cite{kiros2015skip}). Further analyses show that the proposed representations fare better at many of the representation quality tasks described in~\citet{conneau2018you}, showing that they also capture many of the syntactic and semantic considerations expected of good sentence encodings.

In summary, this paper makes the following  contributions:
1) Introduces fake sentence detection as an unsupervised training task for learning sentence encoders that can distinguish between small changes in mostly similar sentences.
2) An empirical evaluation on multiple sentence-level tasks showing representations trained on the fake sentence tasks outperform a strong baseline model trained on language modeling tasks, even when training on small amounts of data (1M vs. 64M sentences) reducing training time from weeks to within 20 hours.




